Shoal: Improving DAG-BFT Latency And Robustness

The Narwhal system is a state-of-the-art Byzantine fault-tolerant scalable architecture that involves constructing a directed acyclic graph (DAG) of messages among a set of validators in a Blockchain network. Bullshark is a zero-overhead consensus protocol on top of the Narwhal's DAG that can order over 100k transactions per second. Unfortunately, the high throughput of Bullshark comes with a latency price due to the DAG construction, increasing the latency compared to the state-of-the-art leader-based BFT consensus protocols. We introduce Shoal, a protocol-agnostic framework for enhancing Narwhal-based consensus. By incorporating leader reputation and pipelining support for the first time, Shoal significantly reduces latency. Moreover, the combination of properties of the DAG construction and the leader reputation mechanism enables the elimination of timeouts in all but extremely uncommon scenarios in practice, a property we name Prevalent Responsiveness" (it strictly subsumes the established and often desired Optimistic Responsiveness property for BFT protocols). We integrated Shoal instantiated with Bullshark, the fastest existing Narwhal-based consensus protocol, in an open-source Blockchain project and provide experimental evaluations demonstrating up to 40% latency reduction in the failure-free executions, and up-to 80% reduction in executions with failures against the vanilla Bullshark implementation.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -pdf -f -e '$$pdflatex=q/pdflatex %O %S/' $<

fast:
	pdflatex $(FILE)


clean:
	for ext in aux log toc lof lot lol dlog bbl \
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) *.d

read: all
	open $(FILE).pdf


==> sections/further.tex <==
\section{Further theoretical improvement}
With pipelining, \sysname introduces an anchor in every round. 
As a result, in the best case, each anchor requires 2 rounds to commit and while non-anchor vertices require 3 rounds.

In this section, we present an approach to further optimize the latency for non-anchor vertices.
In designing \sysname, we have crucially relied on the technique of retrospectively re-interpreting the DAG structure.
Taking this further, we could iterate over the vertices in each round in a deterministic order and treat each vertex as an anchor.
More specifically, for each vertex $v$, we can run an instance of the underlying protocol $\mathcal{P}$ (i.e., DAG-Rider, Tusk, and Bullshark) as a single-shot agreement with $v$ being the first anchor.
If $v$ is ordered by $\mathcal{P}$, we order it.
Otherwise, we skip.
In both cases, we ignore all other ordered/skipped anchors in this instance and move to the next vertex.
For every vertex $v$ we decide to order, we also order the previously skipped vertices in $v$'s causal history.
A pseudocode appears in Algorithm~\ref{alg:bounus}.

\begin{algorithm}
\caption{Single-shot Narwhal-based agreement for each vertex}
\begin{algorithmic}[1]
        \State $r \gets 0$
        \While{\emph{true}}
            \For{\textbf{each} validator $k$}
                \State let $v_{r,k}$ be a vertex by validator $k$ in round $r$
                \State let $F_{r,k}: R \rightarrow A$ be a known to all mapping from 
                \Statex \hspace{9.5mm} rounds to anchors such that $F_{r,k}(r) = k$
                \State execute $\mathcal{P}$, select anchors by $F_{r,k}$, starting from 
                \StateX\hspace{4.5mm} $r$ until the first ordered (not skipped) anchor $A$ 
                \StateX\hspace{4.5mm} is determined.
                \If $A = v_{r,k}$
                    \State order $A$'s causal history according to $\mathcal{P}$ 
                \EndIf
            \EndFor
        \State $r \gets r+1$ 

        \EndWhile
    
\end{algorithmic}
\label{alg:bounus} 
\end{algorithm}

In the theoretical best case, each vertex can be ordered in 2 rounds. 
However, in practice, some validators may be slower and, therefore, require more rounds.
This is because their corresponding single-shot instances would not be able to order them based on the "votes" in the subsequent round, and thus more rounds will be required to determine whether they should be skipped or ordered.
The issue arises because validators must process the vertices in a predetermined deterministic order. Consequently, each vertex that necessitates more rounds incurs a latency penalty for the subsequent vertices.

\sasha{figure?}

\paragraph{Combining with leader reputation}
The above issue can potentially be mitigated by combining it with the leader reputation mechanism.
That is, instead of running a single-shot agreement for every vertex, we can run it for vertices corresponding to responsive validators.
The rest of the vertices can be ordered based on causal history as previously. 
this way, in the best case, vertices corresponding to responsive validators will be ordered in 2 rounds and the rest in 3.
The worst case will become less likely.

